Deep Learning Framework for Hybrid Analog-Digital Signal Processing in mmWave Massive-MIMO Systems

Hybrid analog-digital signal processing (HSP) is an enabling technology to harvest the potential of millimeter-wave (mmWave) massive-MIMO communications. In this paper, we present a general deep learning (DL) framework for efficient design and implementation of HSP-based massive-MIMO systems. Exploiting the fact that any complex matrix can be written as a scaled sum of two matrices with unit-modulus entries, a novel analog deep neural network (ADNN) structure is first developed which can be implemented with common radio frequency (RF) components. This structure is then embedded into an extended hybrid analog-digital deep neural network (HDNN) architecture which facilitates the implementation of mmWave massive-MIMO systems while improving their performance. In particular, the proposed HDNN architecture enables HSP-based massive-MIMO transceivers to approximate any desired transmitter and receiver mapping with arbitrary precision. To demonstrate the capabilities of the proposed DL framework, we present a new HDNN-based beamformer design that can achieve the same performance as fully-digital beamforming, with reduced number of RF chains. Finally, simulation results are presented confirming the superiority of the proposed HDNN design over existing hybrid beamforming schemes.

==> csnameendcsname.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\@setckpt{csnameendcsname\protect \relax \relax \math@bgroup \def 7{7}\def 7{0}\mathgroup \symAMSb \relax \egroup \endcsname {C}$}{
\setcounter{page}{10}
\setcounter{equation}{1}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{section}{2}
\setcounter{subsection}{1}
\setcounter{subsubsection}{1}
\setcounter{paragraph}{0}
\setcounter{IEEEsubequation}{0}
\setcounter{figure}{1}
\setcounter{table}{0}
\setcounter{IEEEbiography}{0}
\setcounter{parentequation}{0}
\setcounter{Item}{0}
\setcounter{Hfootnote}{0}
\setcounter{bookmark@seq@number}{6}
\setcounter{float@type}{4}
\setcounter{AlgoLine}{0}
\setcounter{algocfline}{0}
\setcounter{algocfproc}{0}
\setcounter{algocf}{0}
\setcounter{caption@flags}{0}
\setcounter{continuedfloat}{0}
\setcounter{subfigure}{0}
\setcounter{subtable}{0}
\setcounter{@todonotes@numberoftodonotes}{0}
\setcounter{Changes@AuthorCount}{1}
\setcounter{Changes@Author}{0}
\setcounter{Changes@addedCount}{0}
\setcounter{Changes@deletedCount}{0}
\setcounter{Changes@replacedCount}{0}
\setcounter{Changes@highlightCount}{0}
\setcounter{Changes@commentCount}{0}
\setcounter{authorcommentcount}{0}
\setcounter{ALC@unique}{0}
\setcounter{ALC@line}{0}
\setcounter{ALC@rem}{0}
\setcounter{ALC@depth}{0}
\setcounter{theorem}{0}
\setcounter{lemma}{0}
\setcounter{proposition}{0}
\setcounter{rmk}{0}
\setcounter{section@level}{3}
}

